Generalized Bayesian Posterior Expectation Distillation for Deep Neural Networks

In this paper, we present a general framework for distilling expectations with respect to the Bayesian posterior distribution of a deep neural network classifier, extending prior work on the Bayesian Dark Knowledge framework. The proposed framework takes as input "teacher" and student model architectures and a general posterior expectation of interest. The distillation method performs an online compression of the selected posterior expectation using iteratively generated Monte Carlo samples. We focus on the posterior predictive distribution and expected entropy as distillation targets. We investigate several aspects of this framework including the impact of uncertainty and the choice of student model architecture. We study methods for student model architecture search from a speed-storage-accuracy perspective and evaluate down-stream tasks leveraging entropy distillation including uncertainty ranking and out-of-distribution detection.

==> archived_sections/intro_v1.tex <==
\section{Introduction}

Deep learning models have shown promising results in the areas of computer vision, natural language processing and speech recognition, surpassing the performance of its counterparts as well as human-level \cite{graves2013hybrid, graves2013speech, krizhevsky2012imagenet}. However, the efficacy of such models is largely dependent of vast amounts of labeled data. Neural networks are also known to produce over-confident results (sometimes, even without adverserial inputs) which can be dangerous in more serious applications like medical imaging, self-driving cars, etc. Among all the techniques to overcome these challenges, we turn our focus to Bayesian Inference. In Bayesian Inference, we utilize the Bayes theorem to obtain the posterior distribution over the parameters of our given model. For a given model, let the parameter set be denoted as  $\theta$, and the training set $\pazocal{D} = \{(\mathbf{x_i}, y_{i})\}_{i=1} ^ N$, where each $\mathbf{x}_i$ denotes a $d$-dimensional feature input corresponding to the input indexed at $i$ and $y_i$ denotes an integer for a classification problem or a continuous real value for a regression problem. The prior distribution over the parameter set is denoted as $p(\theta)$. Thus, we obtain the posterior distribution as 
\begin{equation}
    \label{eq:posterior}
    p(\theta|\pazocal{D}) = \frac{p(\pazocal{D}|\theta)p(\theta)}{\int p(\pazocal{D}|\theta)p(\theta) d\theta}
\end{equation}
Ultimately, we obtain the posterior predictive distribution as following:
\begin{equation}
\label{eq:posterior_predictive}
p(y| \mathbf{x}, \pazocal{D}) = \int p(y|\mathbf{x}, \theta) p(\theta|\pazocal{D}) d\theta
\end{equation}
The challenging part in the process of obtaining a posterior predictive distribution is that the integral term (also known as evidence) in equation \ref{eq:posterior} is not always analytically tractable. There are existing methods in the area of variational learning and markov chain monte carlo (MCMC) based sampling techniques to circumvent this challenge. In this study, we focus on a technique that stems out of the combination of an MCMC based sampling technique and knowledge distillation for neural networks \cite{balan2015bayesian, welling2011bayesian, hinton2015distilling}. This technique aims to produce a posterior predictive distribution using a single neural network model of the same size and architecture as the model of our choice, trained using multiple parameter samples from the approximate posterior distribution. We employ this method to the task of classifying where a portion of the pixels have been masked out.  Another way to interpret this task is to think of it as classifying images under occlusion or classifying data points with missing values. Since both these applications are of particular use in practical scenarios, it becomes all the more important to analyze the performance of this method on tasks like these. As we see in the experimental sections of the paper, knowledge distillation into a model of same size, doesn't lead to the same level of performance as the monte carlo estimate of equation \ref{eq:posterior_predictive} obtained using all the samples generated from the approximate posterior distribution. Finally, as an attempt to mitigate this gap, we suggest that increasing the model capacity can further lead to a decrease in the performance gap. We verify this proposition using additional experiments. 


==> archived_sections/related_work_v1.tex <==
\section{Related Work}
In cases where the posterior distribution is not analytically tractable, we try to approximate it. Of all the techniques present in the literature for bayesian neural networks, variational inference (VI) and MCMC based sampling methods have been more popular than the rest \cite{jordan1999introduction, Neal:1996:BLN:525544, welling2011bayesian}. In VI, we define an auxiliary distribution of our choice $q_{\phi} (\theta)$, parameterised by $\phi$ to approximate the true posterior $p(\theta | \pazocal{D})$. The reason for doing this is to get an approximation which can be plugged in the place of $p(\theta | \pazocal{D})$ in equation \ref{eq:posterior_predictive}. Next, we optimize the Kullback-Leibler (KL) divergence between $q_{\phi} (\theta)$ and $p(\theta | \pazocal{D})$:
\begin{equation}
\textrm{KL}(q_{\phi} (\theta) || p(\theta | \pazocal{D})) = \int q_{\phi}(\theta) \log \frac{q_{\phi}(\theta)}{p(\theta | \pazocal{D})}
\end{equation}
Upon further simplification, we obtain that minimizing the KL divergence is equivalent to maximising the following objective:
\begin{equation}
\pazocal{L(\phi)} = \int q_{\phi}(\theta) \log p(\pazocal{D}| \theta) d\theta - \textrm{KL} (q_{\phi}(\theta) || p(\theta))
\end{equation}
This is also known as the evidence lower bound (ELBO) loss. For tractable integral in the first term of our ELBO term, we would typically want a simpler distribution parameterised in $\phi$. However, a simpler distribution doesn't align well with the true posterior and thus, this creates a trade-off between the expressive power of $q_{\phi}(\theta)$ and ease of computation. Another closely related technique is expectation propogation (EP) \cite{minka2001expectation}. The main difference between VI and EP is that in VI, we minimize the $\textrm{KL}(q_{\phi} (\theta) || p(\theta | \pazocal{D}))$, while in EP we minimize $\textrm{KL}(p(\theta | \pazocal{D}) || q_{\phi} (\theta))$. While these methods are useful to obtain an approximate parameterised posterior distribution, they present some challenges when employed in their conventional form. First, the computation cost scales with the amount of data. Secondly, variational methods have a mode-seeking behaviour and this can also lead to a poor approximation of the distribution. A more recent approach has been proposed to tackle the second problem which is known as probabilistic backpropagation (PBP). PBP assumes an already factorised structure for the posterior distribution suitable for tractability in equation \ref{eq:posterior_predictive} and then directly optimizes the posterior predictive distribution to find the parameters of the factorised distribution \cite{hernandez2015probabilistic}. \\
The other line of work extends on MCMC based sampling techniques. Of all the techniques present in the literature, stochastic gradient langevin dynamics (SGLD) \cite{welling2011bayesian} is of primary interest to our study. \emph{Bayesian Dark Knowledge} uses SGLD  to sample from the approximate posterior distribution to train a teacher neural network. Next, we aim to train a student neural network which approximates the bayesian predictive distribution of the teacher neural network. Before we outline the method proposed in, we establish some more notation. Let $p(\theta| \lambda)$ define the prior distribution over the teacher's model parameters $\theta$, parameterised by $\lambda$. In this case, the prior distribution is spherical gaussian distribution centered at $0$ and having precision as $\lambda$. We define the softmax outputs from teacher model using parameters $\theta$ as $p(y_i|\mathbf{x_i}, \theta)$. Next, we define $\pazocal{S}$ as a minibatch of size M drawn from $\pazocal{D}$. Let the total number of training samples in $\pazocal{D}$ be denoted as $N$. $\theta_t$ denotes the parameter set sampled for teacher model at sampling iteration $t$, while $\eta_t$ denotes the learning rate for teacher model at iteration $t$. The langevin noise here is denoted as $z_t \sim \pazocal{N}(0, \eta_t I )$.  Thus, the sampling step for SGLD can be written as:
\begin{equation}
\theta_{t+1} = \theta_{t}+\frac{\eta_{t}}{2}\left(\nabla_{\theta} \log p(\theta | \lambda)+\frac{N}{M} \sum_{i \in \pazocal{S}} \nabla_{\theta} \log p\left(y_{i} | x_{i}, \theta_{t}\right)\right)+ z_{t}
\end{equation}
At this point, let us generate another batch of samples $\pazocal{D'}$ which are used to train the student neural network. One way to obtain $\pazocal{D'}$ by adding gaussian noise of small magnitude to $\pazocal{S}$. The samples from $\pazocal{D'}$ are denoted as $\{(\mathbf{x'_{i}}, y'_{i})\}$. The predictive posterior distribution over $\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}$ using teacher model with parameter set $\theta_{t+1}$ is given as $p(y'_i|\mathbf{x'_i}, \theta_{t+1})$. Similarly, the 
predictive distribution for a student model parameterised by $\omega_t$ is given as $S(y'_i|\mathbf{x'_i}, \omega_t)$. We define the cross-entropy loss between predictive distributions of teacher and student at iteration $t+1$ as
\begin{align*}
\pazocal{L}( \omega_t| \pazocal{D}', \theta_{t+1}) = -\sum_{\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}} \sum_{k=1}^{K} p(y'_i = k|\mathbf{x'_i}, \theta_{t+1}) \log S(y'_i = k|\mathbf{x'_i}, \omega_t)
\end{align*}
At this point, we minimize the above loss by making one optimization update to obtain $\omega_{t+1}$. After all the optimization iterations, we utilize the final parameter set obtained for the student model to make predictions. In the experiments performed by \cite{balan2015bayesian}, they utilize the MNIST dataset with fully-observed images. We argue that the task of classifying MNIST images is relatively easy as a fully connected network used by them achieves a log-likelihood of $1.271 \pm 0.0126$ on test set while trained on 50,000 images. Thus, to analyse this method in more detail, we run extensive experiments on MNIST dataset with masked inputs. 

==> archived_sections/related_work_v2.tex <==
\section{Related Work}
In cases where the posterior distribution is not analytically tractable, we try to approximate it. Some of the previous work done in this direction adapts on the line VI and markov chain monte carlo (MCMC) based sampling methods \cite{jordan1999introduction, Neal:1996:BLN:525544, welling2011bayesian}. In VI, we define an auxiliary distribution of our choice $q_{\phi} (\theta)$, parameterised by $\phi$ to approximate the true posterior $p(\theta | \pazocal{D})$. Next, we optimize the Kullback-Leibler (KL) divergence between $q_{\phi} (\theta)$ and $p(\theta | \pazocal{D})$. \cite{hinton1993keeping} presented the first study to apply VI for neural networks. However, the method presented scalability issues, and to tackle those issues, \cite{graves2011practical} presented an approach using stochastic VI. Another related approach to VI is expectation propagation (EP) \cite{minka2001expectation}. The main difference between VI and EP is that in VI, we minimize the $\textrm{KL}(q_{\phi} (\theta) || p(\theta | \pazocal{D}))$, while in EP we minimize $\textrm{KL}(p(\theta | \pazocal{D}) || q_{\phi} (\theta))$. \citet{soudry2014expectation} shows an online EP algorithm for neural networks with the flexibility of continous weights as well as discrete weights. Another related approach is probabilistic backpropagation (PBP) \cite{hernandez2015probabilistic}. In PBP, we define a parameterised distribution over all the layers over neural network and backpropagate by computing the gradient of the marginal log-likelihood  w.r.t. these parameters. A common problem though with EP and PBP is that they use a diagonal gaussian structure for approximating the posterior distribution. This does not model complex relationships between parameters in the model. To tackle this problem, \citet{louizos2017multiplicative} introduced the concept of \emph{Multiplicative Normalizing Flows}. Under \emph{Multiplicative Normalizing Flows}, we apply a chain of transformations to parameters sampled from our approximate posterior $q_{\phi}(\theta)$, using some additional learnable parameters $\omega$. This technique helps us create samples imitating more complex distributions than the standard mean-field inference. However, this requires the flow to be invertible.

The other line of work extends on MCMC based sampling techniques to sample from approximate posterior distribution and get a monte carlo average of equation \ref{eq:posterior_predictive}. One of the earliest studies in this line of work utilizes Hamiltonian Monte Carlo (HMC) \cite{Neal:1996:BLN:525544} for neural networks. The bottleneck with this method is that it utilizes the full dataset for computing the gradient, subjecting it to scalability issues. This issue has been targeted by stochastic gradient based MCMC algorithms like stochastic gradient langevin dynamics (SGLD) \cite{welling2011bayesian}. SGLD can be seen as fusion of the original SGD algorithm and langevin dynamics. Under SGLD, the earlier iterations of training are used to reach a local mode and then the langevin noise is used to sample around the local mode. \emph{Bayesian Dark Knowledge} \cite{balan2015bayesian} uses SGLD  to sample from the approximate posterior distribution to train a teacher neural network. Next, it aims to train a student neural network which approximates the bayesian predictive distribution of the teacher neural network. With the advent of \emph{Generative Adverserial Networks} \cite{goodfellow2014generative}, there has been some effort behind generative processes for posterior sampling. \citet{wang2018adversarial} introduces a method of distilling the posterior distribution to a generative process, which can be trained in an adverserial fashion. \citet{wang2018adversarial} utilizes the samples generated from SGLD to train a generator. Thus, at test time, rather than running SGLD, posterior samples are generated using the GAN. This approach gives flexibility in terms of computational budget while doing bayesian inference. Another related approach is proposed by \citet{henning2018approximating} where they train a hypernetwork using adverserial training regime. Their method varies slightly from that of \citet{wang2018adversarial} in the sense that the discriminator has to differentiate between pairs of the original input and two possible outputs: one obtained via posterior predictive distribution generated using SGLD and another generated using the GAN. A major difference between \emph{Bayesian Dark Knowledge} and GAN based distillation methods is that the latter set of methods still rely on generating samples for at test time, while the former requires just a single forward pass through the student neural network to produce an estimate of $p(y|\mathbf{x}, \pazocal{D})$. And finally, there's some work which doesn't exactly fit as extensions of VI, EP or MCMC based methods \cite{gal2016dropout, lakshminarayanan2017simple}. \citet{gal2016dropout} suggests a method of quantifying uncertainty by using \emph{dropout} \cite{srivastava2014dropout} at the time of test as well. This method has been termed as MC-dropout and it requires multiple forward passed to get uncertainty in the output. \citet{lakshminarayanan2017simple} implements a simple and scalable technique of utilizing an  ensemble of deep neural networks using proper scoring rules. It uses adverserial style of training to smoothen predictive distributions.

Now, we take a closer look at the distillation technique proposed by \citet{balan2015bayesian}. Before we outline the method proposed in, we establish some more notation. Let $p(\theta| \lambda)$ define the prior distribution over the teacher's model parameters $\theta$, parameterised by $\lambda$. In this case, the prior distribution is a spherical gaussian distribution centered at $0$ with precision denoted as $\lambda$. Next, we define $\pazocal{S}$ as a minibatch of size M drawn from $\pazocal{D}$. Let the total number of training samples in $\pazocal{D}$ be denoted as $N$. $\theta_t$ denotes the parameter set sampled for teacher model at sampling iteration $t$, while $\eta_t$ denotes the learning rate for teacher model at iteration $t$. The langevin noise here is denoted as $z_t \sim \pazocal{N}(0, \eta_t I )$.  Thus, the sampling update for SGLD can be written as:
\begin{equation}
\Delta \theta_{t+1} \!=\!\frac{\eta_{t}}{2}\!\left(\!\nabla_{\theta} \log p(\theta | \lambda)\!+\!\frac{N}{M} \sum_{i \in \pazocal{S}} \nabla_{\theta} \log p\left(y_{i} | x_{i}, \theta_{t}\right)\!\right)+ z_{t}.
\end{equation}
At this point, we generate another batch of samples $\pazocal{D'}$ which are used to train the student neural network. $\pazocal{D'}$ is obtained by adding gaussian noise of small magnitude to $\pazocal{S}$. The samples from $\pazocal{D'}$ are denoted as $\{(\mathbf{x'_{i}}, y'_{i})\}$. The predictive distribution over $\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}$ using teacher model with parameter set $\theta_{t+1}$ is given as $p(y'_i|\mathbf{x'}_i, \theta_{t+1})$. Similarly, the 
predictive distribution for a student model parameterised by $\omega_t$ is given as $S(y'_i|\mathbf{x'}_i, \omega_t)$. The objective for student model is  $\pazocal{L}( \omega_t| \pazocal{D}', \theta_{t+1}) = \sum_{\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}}\textrm{KL}(S(y'_i|\mathbf{x'_i}, \omega_t) || p(y'_i|\mathbf{x'}_i, \theta_{t+1}))$ and run a single optimization iteration to obtain $\omega_{t+1}$. We run this process of sequentially obtaining $\theta_{t+1}$ and $\omega_{t+1}$ until we converge. 


% We define the cross-entropy loss between predictive distributions of teacher and student at iteration $t+1$ as
% \begin{align*}
% &\pazocal{L}( \omega_t| \pazocal{D}', \theta_{t+1}) = \\
% &\quad-\!\!\!\!\!\!\sum_{\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}} \sum_{k=1}^{K} p(y'_i = k|\mathbf{x'_i}, \theta_{t+1}) \log S(y'_i = k|\mathbf{x'_i}, \omega_t).
% \end{align*}
% At this point, we minimize the above loss by making one optimization update to obtain $\omega_{t+1}$. After all the optimization iterations, we utilize the final parameter set obtained for the student model to make predictions.

==> cuts.tex <==



The Bayesian Dark Knowledge approach 


However, they pose significant challenges in terms of high training data requirement as well as bring over-confident while making wrong predictions. Bayesian Inference is a fundamental technique to overcome these challenges. In Bayesian Inference, we utilize the Bayes theorem to obtain the posterior distribution over the parameters of our given model. For a given model, let the parameter set be denoted as  $\theta$, and the training set $\pazocal{D} = \{(\mathbf{x}_i, y_{i})\}_{i=1} ^ N$, where each $\mathbf{x}_i \in \mathbb{R}^d$ denotes a $d$-dimensional feature input corresponding to the input indexed at $i$ and $y_i$ denotes an integer for a classification problem or a continuous real value for a regression problem. The prior distribution over the parameter set is denoted as $p(\theta)$. Thus, we obtain the posterior distribution as 
\begin{equation}
    \label{eq:posterior}
    p(\theta|\pazocal{D}) = \frac{p(\pazocal{D}|\theta)p(\theta)}{\int p(\pazocal{D}|\theta)p(\theta) d\theta}
\end{equation}
Ultimately, we obtain the posterior predictive distribution as following:
\begin{equation}
\label{eq:posterior_predictive}
p(y| \mathbf{x}, \pazocal{D}) = \int p(y|\mathbf{x}, \theta) p(\theta|\pazocal{D}) d\theta
\end{equation}
The challenging part here is that the integral term (also known as evidence) in equation \ref{eq:posterior} is not always analytically tractable. There are existing methods to circumvent this problem based on variational inference (VI), markov chain monte carlo (MCMC) methods, and more recently GAN based methods to approximate the posterior distribution. Among all these methods, the focus of our study is \emph{Bayesian Dark Knowledge}. 

A key advantage of \emph{Bayesian Dark Knowledge} over its counterparts is that it performs ``distillation" of the approximate posterior predictive distribution to a single compact model. At the time of testing, it requires only a single forward pass through the trained ``student" model to approximate equation \ref{eq:posterior_predictive}. A useful application of this can be in low-latency embedded systems where we wish to account for uncertainty without having to store parameter samples or performing multiple forward-passes through a model as required by some other techniques. While the idea is promising, the experimental validations by \cite{balan2015bayesian} are not robust. The experimental validations done on fully observed MNIST dataset for the classification problem point to the fact that there is a low posterior uncertainty in the first place, as evident from the high log-likelihood values on the test set.  Thus, the performance of the technique remains untested against other higher levels of posterior uncertainty. We aim to address this issue through our study. The main goal of this paper is to evaluate the method of \emph{Bayesian Dark Knowledge} under different levels of posterior uncertainty. As we see in the later sections of the paper, we find that the original claim made by \citet{balan2015bayesian} of distilling the posterior predictive distribution to a student model of the same size doesn't hold true. We further show that increasing the model capacity can help mitigate this performance gap to some extent.

-----------------

And finally, there's some work which doesn't exactly fit as extensions of VI, EP or MCMC based methods \cite{gal2016dropout, lakshminarayanan2017simple}. \citet{gal2016dropout} suggests a method of quantifying uncertainty by using \emph{dropout} \cite{srivastava2014dropout} at the time of test as well. This method has been termed as MC-dropout and it requires multiple forward passed to get uncertainty in the output. \citet{lakshminarayanan2017simple} implements a simple and scalable technique of utilizing an  ensemble of deep neural networks using proper scoring rules. It uses adverserial style of training to smoothen predictive distributions.

Now, we take a closer look at the distillation technique proposed by 


% We define the cross-entropy loss between predictive distributions of teacher and student at iteration $t+1$ as
% \begin{align*}
% &\pazocal{L}( \omega_t| \pazocal{D}', \theta_{t+1}) = \\
% &\quad-\!\!\!\!\!\!\sum_{\{(\mathbf{x'_i}, y'_i)\} \in \pazocal{D'}} \sum_{k=1}^{K} p(y'_i = k|\mathbf{x'_i}, \theta_{t+1}) \log S(y'_i = k|\mathbf{x'_i}, \omega_t).
% \end{align*}
% At this point, we minimize the above loss by making one optimization update to obtain $\omega_{t+1}$. After all the optimization iterations, we utilize the final parameter set obtained for the student model to make predictions.






introduces a method of distilling the posterior distribution to a generative process, which can be trained in an adverserial fashion. \citet{wang2018adversarial} uses the samples generated from SGLD to train a generator. Thus, at test time, rather than running SGLD, posterior samples are generated using the GAN. 

Another related approach is proposed by \citet{henning2018approximating} where they train a hypernetwork using an adverserial training regime. Their method varies slightly from that of \citet{wang2018adversarial} in the sense that the discriminator has to differentiate between pairs of the original input and two possible outputs: one obtained via posterior predictive distribution generated using SGLD and another generated using the GAN. A major difference between \emph{Bayesian Dark Knowledge} and GAN based distillation methods is that the latter set of methods still rely on generating samples for at test time, while the former requires just a single forward pass through the student neural network to produce an estimate of $p(y|\mathbf{x}, \pazocal{D})$. 

==> experiment_masked_MNIST.tex <==
\section{Assessing  Robustness to Uncertainty}
As noted in the introduction, the original empirical investigation of Bayesian Dark Knowledge for classification focused on the MNIST data set. However, the models fit to the MNIST data set have very low posterior uncertainty and we argue that it is thus a poor benchmark for assessing the performance of Bayesian Dark Knowledge. In this section, we investigate two orthogonal modifications of the standard MNIST data  set: reducing the training set size and masking regions of the input images. Our goal is to produce a range of benchmark problems with varying posterior predictive uncertainty. 

\textbf{Data Set Manipulations:} The full MNIST dataset consists of 60,000 training images and 10,000 test images, each of size $28 \times 28$, distributed among 10 classes \cite{lecun1998mnist}. As a first manipulation, we consider sub-sampling the labeled training data to include 10,000, 20,000, 30,000 or all 60,000 data cases when performing posterior sampling for the teacher model. Importantly, we use all 60,000 unlabeled training cases in the distillation process, which does not require labeled instances. This allows us de-couple the impact of reduced labeled training data on posterior predictive distributions from the effect of the amount of unlabeled data available for distillation.

As a second manipulation, we generate images with occlusions by randomly masking out parts of each available training and test image. For generating such images, we randomly choose a square $m\times m$ region (mask) and set the value for pixels in that region to 0. Thus, the masking rate for a $28 \times 28$ MNIST image corresponding to the mask of size $m\times m$ is given by $r = \frac{m \times m}{28 \times 28}$. We illustrate original and masked data in Figure \ref{fig:mnist}. We consider a range of square masks resulting in masking rates between 0\% and 86.2\%.
\begin{figure}[!htbp]
    \centering
    \subfigure[Original images]{\includegraphics[width=0.18\textwidth]{figures/unmasked_images.pdf}}
    \hspace{1cm}
    \subfigure[Processed images]{\includegraphics[width=0.18\textwidth]{figures/masked_images.pdf}}
    \caption{Inputs after data pre-processing step with $m=14$.\vspace{-1em}}
    \label{fig:mnist}
\end{figure}

\textbf{Models:} We use a fully-connected neural network of architecture $784-400-400-10$ for both teacher and student with $ReLU$ non-linearities at the hidden layers. The only addition we make to the student model is using dropout layers for regularization. We run the distillation procedure using the following hyperparameters: fixed teacher learning rate $\eta_t = 4 \times 10^{-6}$, teacher prior precision $\lambda = 10$, initial student learning rate $\rho_t = 10^{-3}$, student dropout rate $p=0.5$, burn-in iterations $B=1000$, thinning interval $\tau = 100$, and total training iterations $T= 10^6$. For training the student model, we use the \emph{Adam} algorithm and set a learning schedule for the student such that it halves its learning rate every 100 epochs. For computing the teacher model's performance on the test set, we use all samples after burn-in  and average the softmax outputs generated by each sample. For the student model, we use the final model obtained after training. We consider the negative log-likelihood (NLL) on the test set as a metric for model performance (zero is the minimum possible value). 

\textbf{Results:} The NLL of the teacher for different labeled training data set sizes and masking rates is shown in Figure \ref{fig:delta_plot}(left) along with the difference between the NLL using the student and teacher in Figure \ref{fig:delta_plot}(right).%\footnote{The detailed results from the experiments are given in Table \ref{tab:masked_mnist_results} present in the Appendix A.} \\
\begin{figure*}[!htbp]
    \centering
    \subfigure{\includegraphics[width=0.4\textwidth]{figures/teacher_nll_missingness_results.pdf}}
    \subfigure{\includegraphics[width=0.4\textwidth]{figures/missingness_results.pdf}}
    % \caption{(a)  (b) }
    \caption{Left: NLL on test set using teacher model. Right: Difference in NLL on test set between student and teacher.}
    \label{fig:delta_plot}
\end{figure*}
As we can see, the teacher obtains very low NLL values when the data set is at full size and no masking is applied, which replicates the results shown by \citet{balan2015bayesian}. As the amount of labeled training data decreases, the NLL generally increases, but only slowly. On the other hand, as the masking rate increases, the NLL of the teacher increases to nearly the maximum possible value, indicating that the posterior predictive distribution is approximately uniform. 

Next,  we consider the gap between the teacher ensemble and the student model. First, we see that the gap is very low for the case of no  masking and 60,000 training instances, again replicating the results of \citet{balan2015bayesian}. We can also see that the gaps between the teacher and the student become much larger for intermediate masking rates. However, we note that the gap in performance between the student and the teacher is not monotonically increasing with the masking rate. The reason for this is that as the masking rate goes to one, we can see from Figure 2(left) that the the posterior predictive distribution becomes very close to uniform. It is in fact very easy for the student to learn to output the uniform distribution for every input  image, so the gap between the teacher and the student becomes minimal. 

The primary conclusion of this experiment is that compression of the full posterior predictive distribution into a student model of the same capacity as the teacher network is failing under some experimental conditions. Specifically, the original Bayesian Dark Knowledge approach appears  to not be robust to the impact that the masking operation has on posterior predictive uncertainty. We perform additional experiments on convolutional models and present a similar set of results in Appendix A. Appendix A also includes posterior predictive entropy plots verifying the effect of masking on posterior uncertainty. 



%Under such low NLL, we can interpret that the teacher will concentrate most of the probability on the true class. This makes the distillation process somewhat easier as at that point, the cross-entropy loss between teacher and student tends to move towards a binary-cross entropy loss where true labels are generated by the teacher model. We already know that this task is easier as we witness the teacher model learning well under such objective. Next, we consider the case when the masking rate is extremely high (e.g. 0.862). At this point, since the model doesn't observe anything meaningful except dark pixels, the posterior predictive distribution would flatten out and develops a tendency to predict all the classes with equal probability. Since, it's easier to imitate a flat posterior predictive distribution, the student's performance is very similar to the teacher and thus the gap in performance is low. As we would expect, the performance of a teacher model doesn't improve with the increasing number of training samples as none of them have any meaningful information. The case becomes interesting as we look at the range of masking rates in between the extremes. Consider the case where the masking rate is set to 0.413. At this point, there's some amount of information visible in the image and thus it wouldn't cause a collapse in the posterior predictive distribution. Also, since the masking in the images is at random, having more images in the training set will help in better learning for the model. This is clearly evident from Figure \ref{fig:delta_plot} (a), where we have lower values of NLL loss as we increase the value of $N$ for missing rate as 0.413. The distillation becomes harder at this point as the posterior predictive distribution becomes more complex compared to the degenerate cases discussed previously, and this affects the performance of the student. As we can see in Figure \ref{fig:delta_plot} (b), the gap in NLL loss rises for intermediate values of missing rate.


==> improving_distillation.tex <==
\section{Improving Bayesian Dark Knowledge}

\subsection{Effect of Student Model Capacity on Performance}
In this section, we show that increasing student model capacity can  close some of the performance gap we highlighted in the previous section. We investigate both fully-connected and convolutional models.

\textbf{Fully-Connected Neural Networks:} We first define a base architecture that we leverage to build larger models. The base architecture is a $784-400-400-1$ model, and is also used for the teacher model.
Next, we use a multiplication factor $K$ to multiply the number of units in the hidden layers to generate models of different capacities.  For a given value of $K$, the student model architecture is given by: $784-\floor*{400 \cdot K}-\floor*{400 \cdot K}-1$. We choose the experimental setting of $N=60,000$ and masking rate of $0.25$, as this resulted in a large performance gap in the previous  section. We use the same hyperparameters as stated in the previous section and examine the the performance gaps in distillation as we vary $K$. 

The results for this experiment are shown in Figure \ref{fig:model_expansion_results}(left).
As we can see, the gap between the NLL of student and teacher drops by about $60\%$ as we increase the value of $K$ to 5. This shows that increasing the model capacity helps improve the performance of the student model significantly.

\textbf{Convolutional Neural Networks:}
For CNNs, we follow the same strategy as we did in the case of FCNNs. We define a base architecture and then build on the existing base architecture by increasing the number of filters and hidden units. The base architecture for our CNN model is: Conv(num\_kernels = 10, kernel\_size = 4, stride = 1) - MaxPool(kernel\_size=2) - Conv(num\_kernels = 20, kernel\_size = 4, stride = -1) - MaxPool(kernel\_size=2) - FC (80) - FC (10), and is also used for the teacher model. For increasing the model capacity of student models, we use a multiplication factor of $C$ to multiply the number of kernels in convolutional layers and the number of hidden units for fully connected layer in the base architecture. The new architecture is given as: Conv(num\_kernels = $\floor*{10 \cdot C}$, kernel\_size = 4, stride = 1) - MaxPool(kernel\_size=2) - Conv(num\_kernels = $\floor*{20 \cdot C}$ = , kernel\_size = 4, stride = 1) - MaxPool(kernel\_size=2) - FC ($\floor*{80 \cdot C}$) - FC (10). We again perform our experiment with the setting $N=60,000$ and masking rate of $0.25$ for different values of $C$. The results are shown in the Figure \ref{fig:model_expansion_results}(right).
\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/model_expansion_results.pdf}
    \vspace{-.2in}
    \caption{Comparison of the gap in performance between the student and the teacher for different student model sizes. The left plot shows results for the FCNN. The right plot shows results for CNN.\vspace{-1.5em}}
    \label{fig:model_expansion_results}
\end{figure} 

The gap between the NLL of student and teacher reduces by approximately $60\%$ as we set $C = 3$. This is again a significant improvement in the performance of the student model as compared to the base case where $C = 1$.  

% \subsection{Learning Sparse Student Models}
% In the previous subsection, we saw that increasing model capacity can help reduce the performance gap between the student model and the teacher ensemble. However, increasing the model capacity can lead to a much higher storage and computational cost, which is not usually feasible in the case of low-powered edge devices. A favourable scenario for such restrictive hardware specifications would be to compress these student models even further. To achieve this, we utilize the concept of network pruning to obtain smaller models. In this subsection, we describe two principled methods used in network pruning namely Sparse Structure Learning and Iterative Weight Pruning,  and demonstrate their utility. We also introduce a baseline method of exhaustive search over student models which is similar to the model width multiplication search we did in the previous subsection. \\

% \textbf{Sparse Structure Learning}: Under this method, we look to obtain models which have sparse hidden units and/or sparse channels which can be completely removed to obtain a smaller model. This can be done using Group Lasso Penalty \cite{yuan2006model}, which is a widely used regularization function to set a group of parameters either active or diminishing their magnitudes simultaneously. The formulation of the regularization function can be written as follows:
% \begin{equation}
%     R(\theta) = \lambda \sum_{g=1}^G \sqrt{dim(\theta_g)}  \left \Vert \theta_g \right\Vert_2
% \end{equation}
% Here, $\theta_g$ denotes the parameters of the group, $G$ denotes the total number of groups, $dim(\theta_g)$ denotes the number of parameters in the group, $\left \Vert . \right\Vert_2$ denotes the L2 norm of the group vector, and $\lambda$ denotes the regularization strength. A higher value of $\lambda$ would be more aggressive with the penalty and thus would prune more number of groups. Another thing to note here is the scaling factor $\sqrt{dim(\theta_g)}$, which will scale the penalty according to the number of parameters in the group. The scaling factor is useful because it will penalize the groups with larger number of parameters more as it's harder to get the L2 norm of such groups to diminish to 0 otherwise.

% An important part of the Group Lasso Penalty is the formation of the groups. For fully-connected networks, we prune a neuron in a layer if the magnitude of all the incoming connection weights to the neuron from it's previous layer tend to 0. More formally, if we denote the weight matrix of layer $L$ as $\mathbf{w}^L \in \rm I\!R^{m \times n}$, where the input to layer $L$ has $n$ dimensions and output has $m$ dimensions, then each row of $\mathbf{w}^L$ is considered a single group. As all the weight magnitudes in the vector $w^{L}_{k, :}$ go to zeros, we can effectively prune out the $k^{th}$ neuron in the $(L+1)^{th}$ layer. For convolutional networks, we prune the output channel of a particular convolutional layer if all the weights corresponding to all the input channel kernels simultaneously turn to zeros. In formal notation, if we denote the weight matrix of the 2D convolutional layer $L$ as $\mathbf{w}^L \in \rm I\!R^{i \times o \times h \times w}$, where $i$ denotes the number of input channels, $o$ denotes the number of output channels, $h$ denotes the spatial height, $w$ denotes the spatial width, then $\mathbf{w}^L_{:, k, :, :}$ denotes a group of parameters which correspond to the $k^{th}$ output channel of layer $L$. Thus, if all the weight magnitudes in $\mathbf{w}^L_{:, k, :, :}$ turn to zeros, we can effectively prune out the output channel $k$ and also reduce the number of input channels in the layer $(L+1)$ by one. 

% As we can clearly see, this nature of pruning makes the resulting weight matrices smaller and thus resulting in direct reduction in storage space (num. of parameters) requirements as well as the number of floating point operations (FLOPS) for a forward pass through the network.\\

% \textbf{Iterative Weight Pruning}: 

==> introduction.tex <==
\section{Introduction}

Deep learning models have shown promising results in the areas of computer vision, natural language processing, speech recognition, and more \cite{krizhevsky2012imagenet,graves2013hybrid,graves2013speech}. However, existing point estimation-based training methods for these models may result in predictive uncertainties that are not well calibrated, including the occurrence of confident errors. 

It is well-known that Bayesian inference can often provide more robust posterior predictive distributions in the classification setting compared to the use of point estimation-based training. However, the integrals required to perform Bayesian inference in neural network models are also well-known to be intractable. Monte Carlo methods provide one solution to representing neural network parameter posteriors as ensembles of networks, but this can require large amounts of both storage and compute time. 

To help overcome these problems, \citet{balan2015bayesian} introduced an interesting model training method referred to as \emph{Bayesian Dark Knowledge} that attempts to compress a traditional Monte Carlo approximation to the parameter posterior, represented as an ensemble of teacher networks, into a single student network representing the posterior predictive distribution. Further, the authors show that this approach is successful in the classification setting using a student network whose architecture matches that of a single network in the teacher ensemble. The Bayesian Dark Knowledge method also uses online learning of the student model based on single samples from the parameter posterior per iteration, resulting in a training algorithm that requires only twice as much space as a standard point estimate-based learning procedure. 

While the algorithmic properties and performance of the Bayesian Dark Knowledge method appear very promising in the classification setting based on the results presented by \citet{balan2015bayesian}, these results are limited to the MNIST data set in terms of real data. As can clearly be seen in the original paper, there is very little uncertainty in the posterior predictive distribution on MNIST using the network architecture selected by the authors. As a result, the performance of Bayesian Dark Knowledge in regimes of even moderate posterior predictive uncertainty has not been adequately examined. 

In this work, we examine the robustness of Bayesian Dark Knowledge to higher levels of posterior uncertainty and show that using a student network that matches the teacher architecture may result in a performance gap. Further, we show that the gap between the teacher ensemble and the student can be effectively reduced by increasing the capacity of the student. We examine two methods to  increase posterior predictive uncertainty for the MNIST data set, and present results on both fully connected and convolutional models.



==> methods.tex <==
\section{Methods}
\subsection{Posterior Information Distillation}
Suppose that we define our posterior over the neural network parameters as shown in Equation 1. In this case, from a practical standpoint, we are interested in computing various information while marginalizing over the posterior to account for the uncertainty in the parameters. One of the most common examples of such information is the posterior predictive distribution, which is shown in Equation 2. In the case of standard MCMC methods, this would involve us doing sampling over the parameter posterior distribution and then computing the monte carlo approximation of the expectation as shown in Equation 3.

p\emph{Bayesian Dark Knowledge} \cite{balan2015bayesian} introduces the idea of distilling this information to another neural network model, also known as the student network. The benefit of distillation is that it saves storage space  as we don't have to store parameter posterior samples, as well as computation time as we only need to do one forward pass through the student model. \emph{Bayesian Dark Knowledge} introduces a specific algorithm just for compressing the mean of the posterior predictive distribution. We extend this idea further and develop a framework which can help in distilling other statistics based on the posterior predictive distribution. 

We define a statistic based on the predictive distribution as $g(y|\mathbf{x}, \theta)$. Note that the value of this statistic is dependent on the parameters $\theta$. The expected value of this statistic under the parameter posterior can be written as:

\begin{equation}
    g(y| \mathbf{x}) = \E_{p(\theta | \gD)} \left[ \right]
\end{equation}

\subsection{Network Pruning}
For pruning the student models, we apply Group Lasso regularization. Under this method, we look to obtain models which have sparse hidden units and/or sparse channels which can be completely removed to obtain a smaller model. The formulation of the regularization function can be written as follows:
\begin{equation}
    R(\theta) = \lambda \sum_{g=1}^G \sqrt{dim(\theta_g)}  \left \Vert \theta_g \right\Vert_2
\end{equation}
Here, $\theta_g$ denotes the parameters of the group, $G$ denotes the total number of groups, $dim(\theta_g)$ denotes the number of parameters in the group, $\left \Vert . \right\Vert_2$ denotes the L2 norm of the group vector, and $\lambda$ denotes the regularization strength. A higher value of $\lambda$ would be more aggressive with the penalty and thus would prune more number of groups. Another thing to note here is the scaling factor $\sqrt{dim(\theta_g)}$, which will scale the penalty according to the number of parameters in the group. The scaling factor is useful because it will penalize the groups with larger number of parameters more as it's harder to get the L2 norm of such groups to diminish to 0 otherwise.

An important part of the Group Lasso Penalty is the formation of the groups. For fully-connected networks, we prune a neuron in a layer if the magnitude of all the incoming connection weights to the neuron from it's previous layer tend to 0. More formally, if we denote the weight matrix of layer $L$ as $\mathbf{w}^L \in \rm I\!R^{m \times n}$, where the input to layer $L$ has $n$ dimensions and output has $m$ dimensions, then each row of $\mathbf{w}^L$ is considered a single group. As all the weight magnitudes in the vector $w^{L}_{k, :}$ go to zeros, we can effectively prune out the $k^{th}$ neuron in the $(L+1)^{th}$ layer. For convolutional networks, we prune the output channel of a particular convolutional layer if all the weights corresponding to all the input channel kernels simultaneously turn to zeros. In formal notation, if we denote the weight matrix of the 2D convolutional layer $L$ as $\mathbf{w}^L \in \rm I\!R^{i \times o \times h \times w}$, where $i$ denotes the number of input channels, $o$ denotes the number of output channels, $h$ denotes the spatial height, $w$ denotes the spatial width, then $\mathbf{w}^L_{:, k, :, :}$ denotes a group of parameters which correspond to the $k^{th}$ output channel of layer $L$. Thus, if all the weight magnitudes in $\mathbf{w}^L_{:, k, :, :}$ turn to zeros, we can effectively prune out the output channel $k$ and also reduce the number of input channels in the layer $(L+1)$ by one. 

As we can clearly see, this nature of pruning makes the resulting weight matrices smaller and thus resulting in direct reduction in storage space (num. of parameters) requirements as well as the number of floating point operations (FLOPS) for a forward pass through the network.
